PrivColl: Practical Privacy-Preserving Collaborative Machine Learning

Collaborative learning enables two or more participants, each with their own training dataset, to collaboratively learn a joint model. It is desirable that the collaboration should not cause the disclosure of either the raw datasets of each individual owner or the local model parameters trained on them. This privacy-preservation requirement has been approached through differential privacy mechanisms, homomorphic encryption (HE) and secure multiparty computation (MPC), but existing attempts may either introduce the loss of model accuracy or imply significant computational and/or communicational overhead. In this work, we address this problem with the lightweight additive secret sharing technique. We propose PrivColl, a framework for protecting local data and local models while ensuring the correctness of training processes. PrivColl employs secret sharing technique for securely evaluating addition operations in a multiparty computation environment, and achieves practicability by employing only the homomorphic addition operations. We formally prove that it guarantees privacy preservation even though the majority (n-2 out of n) of participants are corrupted. With experiments on real-world datasets, we further demonstrate that PrivColl retains high efficiency. It achieves a speedup of more than 45X over the state-of-the-art MPC/HE based schemes for training linear/logistic regression, and 216X faster for training neural network.

==> chapters/abstract.tex <==
\begin{abstract}
Machine learning algorithms are widely used in most industries nowadays.
In order to get better outcomes, data owners are tending to collaborative learning - a technique that allows two or more participants, each with its own training dataset, to construct a joint model. 
It is desired that the collaboration should not expose either the private data of each individual owner or the model parameters trained on their datasets. 
While the problem has been approached through the differential privacy mechanisms and paradigms of homomorphic encryption (HE) or secure multiparty computation (MPC), those existing attempts may either introduce loss of model accuracy or imply significant computational or communicational overhead. 
In this work, we present a provably secure and efficient framework named \codename for protecting both training data and the trained model against a honest-but-curious attacker, while ensuring correctness of the training process.
\codename employs share computing techniques for securely evaluating addition operations in a multiparty computation environment, and achieves practicability by removing costly cryptographic implementations such as multiplication and non-linear functions. 
We formally prove that such privacy preservation is guaranteed even though majority of participants are corrupted, conditioned on a sufficiently large rank of training dataset.
With experiments on real-world datasets, we further demonstrate that \codename retains efficiency in large-scale data. 
It achieves a speedup of more than 45X over the state-of-the-art schemes based on MPC or HE for training linear/logistic regression, and 216X faster for training neural network. 
\keywords{Privacy preserving  \and machine learning \and collaborative learning.}
\end{abstract}

==> chapters/background.tex <==
 \section{Background}
\label{sec:background}
\subsection{Gradient Descent Optimization}
First, we briefly introduce necessary background of gradient descent optimization. 
Gradient descent is by far the most common optimization strategy used in machine learning and deep learning at the moment. It is used to find the values of a functions coefficients that minimize a cost function as far as possible. 
In the optimization, a cost function $J(w)$ is defined to learn the coefficient vector $W$, and $W$ is calculated by the optimization $\argmin_w J(w)$, and a coefficient $w_j$ is updated as:
\begin{equation}
w_j := w_j - \alpha\frac{\partial{J(w)}}{\partial{w_j}}
\end{equation}


The cost function $J$ is defined as $J(\sigma(XW), y, W)$, where $\sigma$ is determined by the learning model. For example, in logistic regression, $\sigma$ is usually a sigmoid function $1/(1+e^{-z})$, while in neural network, $\sigma$ is a composite function - known as forward propagation. According to the chain rule in calculus, the gradient with respect to a coefficient $w_j$ is computed as: $\frac{\partial{J}}{\partial{\sigma}}\frac{\partial{\sigma}}{\partial{XW}}\frac{\partial{XW}}{\partial{w_j}} + \tau_j$, where $\tau_j$ is the gradient with respect to the regularization term, which is independent to $X$. Let $\Delta = \frac{\partial{J}}{\partial{\sigma}}\frac{\partial{\sigma}}{\partial{XW}}$ which is a function of $XW$, and $\frac{\partial{XW}}{\partial{w_j}}$ equals to $x_j$, then the gradient with respect to $w_j$ can be written as: 
\begin{equation}
\frac{\partial{J(w)}}{\partial{w_j}} = \Delta x_j + \tau_j
\end{equation}

\subsection{Additive Secret Sharing Scheme}
Secret sharing schemes are used to securely distribute secret values amongst a group of participants. \codename employs the secret sharing scheme proposed by \cite{bogdanov2008sharemind}, which uses \emph{additive sharing} over $\mathbb{Z}_{2^{32}}$, where a secret value $srt$ is split to shares $E^1_{srt},...,E^s_{srt} \in \mathbb{Z}_{2^{32}}$  such that
\begin{equation}
	E^1_{srt}+E^2_{srt}+...+E^s_{srt} \equiv srt \mod 2^{32}
\end{equation}
and any $s-1$ element subset $\{E^{i_1}_{srt},...,E^{i_{s-1}}_{srt}\}$ is uniformly distributed. As a result, participants cannot learn anything about $srt$ unless all of them join their shares.

The scheme has a homomorphic property that allows for efficient secure addition on a set of secret values $srt_1,...,srt_s$. By distributing the secret shares amongst the participants and then simply add the shares individually,  the addition result can be reconstruct without revealing the secret addends.


==> chapters/background1.tex <==
\section{Background}\label{sec:background}
In this section, we introduce the background knowledge that is necessary to understand our framework.

\subsection{Gradient Descent Optimization}
\label{sec:gd}
Gradient descent is by far the most commonly used optimization strategy among various machine learning and deep learning algorithms. 
It is used to find the values of functions coefficients that minimize a cost function as far as possible.
Given a defined cost function $J$,  the coefficient matrix $W$ is derived by the optimization $\argmin_W J$, and is updated as: %\baigd{Complete this sentence. Got lost: what is $j$, when to update?}
\begin{equation}
W := W - \alpha\frac{\partial{J}}{\partial{W}}
\end{equation}

Given a particular training dataset $X$ and a label matrix $y$, the cost function $J$ can be defined as $J(\sigma(XW), y, W)$, %\baigd{contradict $J(w)$ above. What is $X$?}
where $\sigma$ is determined by the learning model. For example, in logistic regression, $\sigma$ is usually a sigmoid function $1/(1+e^{-z})$, while in neural network, $\sigma$ is a composite function that is known as forward propagation. According to the chain rule in calculus, the gradient with respect to $W$ is computed as $\frac{\partial{J}}{\partial{\sigma}}\frac{\partial{\sigma}}{\partial{XW}}\frac{\partial{XW}}{\partial{W}} + \tau$, where $\tau$ is the gradient with respect to the regularization term, which is independent to $X$. Let $\Delta = \frac{\partial{J}}{\partial{\sigma}}\frac{\partial{\sigma}}{\partial{XW}}$, and $\frac{\partial{XW}}{\partial{W}}$ equals to $X$, then the gradient with respect to $W$ can be written as:
\begin{equation}
\label{equ:chain}
\frac{\partial{J}}{\partial{W}} = \Delta X + \tau.
\end{equation}

As such, we can decompose the gradient descent optimization into $\Delta$ , $X$ and $\tau$, in which $\Delta$ is a function of $XW$.  This provides an algorithmic foundation of \codename.  

%\baigd{add one or two sentences to brief how this will be adapted by \codename, or at least let readers know why background is introduced.}

\subsection{Additive Secret Sharing Scheme}
Secret sharing schemes aim to securely distribute secret values amongst a group of participants. \codename employs the secret sharing scheme proposed by \cite{bogdanov2008sharemind}, which uses \emph{additive sharing} over $\mathbb{Z}_{2^{32}}$. 
In this scheme, a secret value $srt$ is split to $s$ shares $E^1_{srt},...,E^s_{srt} \in \mathbb{Z}_{2^{32}}$  such that
\begin{equation}
	E^1_{srt}+E^2_{srt}+...+E^s_{srt} \equiv srt \mod 2^{32}, 
\end{equation}
and any $s-1$ elements $E^{i_1}_{srt},...,E^{i_{s-1}}_{srt}$ are uniformly distributed. \baigd{suggestion: writing should focus on answering readers' potential questions, rather than introducing burden for their memory. Here, the $\{E^{i_1}_{srt},...,E^{i_{s-1}}_{srt}\}$ doesn't give any information---as I don't say it is used anywhere in the remaining sections---but it needs reader to stop to think about its meaning, and to try to memorize this notation. ``any set consisting of $s-1$ shares is uniformly distributed'' reads equivalent. BTW, what does it mean by ``a set is uniformly distributed?''} \yanjun{Below, I added a paragraph to detail how a secret sharing scheme works for addition which might help with a clearer illustration of our workflow in Section 3.3. I also revised the sentence ``any $s-1$ element subset $\{E^{i_1}_{srt},...,E^{i_{s-1}}_{srt}\}$ is uniformly distributed'' to ``any $s-1$ elements $E^{i_1}_{srt},...,E^{i_{s-1}}_{srt}$ are uniformly distributed''}
As a result, the value of $srt$ cannot be derived by any participant who has part of the shares, unless all of them join their shares.
%participants cannot \highlight{learn anything about $srt$} \baigd{this is too informal and vague. ``the value of $srt$ cannot be derived by any participant who has part of the shares, unless all of them join their shares''} unless all of them join their shares.

In addition, the scheme has a homomorphic property that allows for efficient and secure addition on a set of secret values $srt_1,...,srt_s$ held by corresponding participants $S_1,...,S_s$. First, each participant $S_i$ executes a randomised sharing algorithm $Shr(srt_i, S)$ to split the $srt_i$ into shares $E^{1}_{srt_i},...,E^{s}_{srt_i}$, and distribute each of the shares to other participants correspondingly, for example, distribute $E^{j}_{srt_i}$ to $S_j$. Then, each participant $S_i$  individually adds the shares they holds $E^{i}_{srt_1},...,E^{i}_{srt_s}$ and produces $\sum_{j=1}^sE^{i}_{srt_j}$ (denoted by $E^i$ for brevity). After that, a reconstruction algorithm $Rec(\{(E^{i}, S_i)\}_{S_i \in S})$, which simply takes $E^i$ from each participant and add them together, can be executed by an aggregator to reconstruct the $\sum_{i=1}^s srt_i$ without revealing any secret addends $srt_i$.

%By distributing the secret shares amongst the participants and then simply adding the shares individually,  the addition result can be reconstructed without revealing the secret addends.


==> chapters/design.tex <==
\section{Design of \codename}
\label{sec:design}
%In this section, we present the privacy preserving collaborative framework for machine learning algorithms using gradient descent for optimization.


\subsection{Threat Model}
\label{sec:threat}
The involved parties in \codename are a set of local nodes (data owners) $S_1, ..., S_s$, who holds different features of the training samples denoted by $X^l$ $(l \in \{1,...,s\})$  and the corresponding local model $W^l$ $(l \in \{1,...,s\})$ respectively, interacting with an aggregation server $Agg$.

Each $X^l$ is a $m \times d_l$ matrix representing $m$ training samples with $d_l$ features.
In \codename, $m$  is public and known by every party, and $d_l$  is private and only known by the corresponding data owner $S_l$.
Let $X$ be a $m \times n$ matrix to denote the vertical concatenation of the local training datasets $X^1, ..., X^s$, where $n = \sum_{l=1}^{s}d_l$.
Since $d_l$  is private and therefore $n$ (i.e. the number of overall features in $X$) is unknown unless all of local nodes join their views.

We assume an honest-but-curious adversary $\mathcal{A}$, who follows the collaboration protocols and training procedures, but aims to obtain the datasets of other local nodes and/or the model parameters trained out of them.
The adversary may control the aggregation server $Agg$, and $t$ out of $s$ local nodes. Here, we assume $t < s-1$, as the local nodes who collude with $Agg$ will have the knowledge of the \emph{sum} of the intermediate results produced by other honest nodes. Therefore, to achieve the privacy preservation, we need at least $2$ honest local nodes in \codename (Detailed in Section \ref{sec:security}). %\baigd{why isn't it $t<s$?}


\subsection{Definitions of Privacy Preservation and Correctness}
The privacy preservation and functional correctness are the main properties \codename aims to achieve.
Below we present the definition of these two properties.
\begin{definition}
	\label{def:security}
	\textbf{(Privacy Preservation)}
	Under the adversary model, we say that  \codename  preserves privacy if the probability of solving $X^l$ or $W^l$ is negligible $(\leq2^{-128})$  %\baigd{what is considered as negligible? This is a formal definition, so a precise/methamatical presentation is needed}
	for any Probabilistic Polynomial-time (PPT) adversary. %\baigd{what is PPT adversary?}
\end{definition}

\begin{definition}
	\label{def:correct}
	\textbf{(Correctness)}
	Given a function $\mathcal{F}$ which takes as input a training dataset $X$.  A function $\mathcal{F^\prime}$ which takes as input $X^1, ..., X^s$ and each of them is associated with a local node $S_l \in S$. $X$ is the vertical concatenation of the $X^1, ..., X^s$ as defined in Section \ref{sec:threat}.
	%Given a function $\mathcal{F}$ which takes as input a training dataset $X \in \mathbb{R}^{m\times{n}}$, and \highlight{assume $X$ is partitioned into a set of  $X^l$ ($l = [1, ... , s]$),} \baigd{Define them at the first occurrence - section 3.1, and then retrain to redefine them everywhere} and each of them is associated with a local node $S_l \in S$, \highlight{where $S$ is the set of local nodes interacting with an aggregation node $Agg$.}  \baigd{This has been given to readers. Don't repeat it. }
	We say that $\mathcal{F^\prime}$ in  \codename  is \underline{correct}, if $\mathcal{F^\prime}(\{(S_l, X^l), Agg\}_{S_l \in S})=\mathcal{F}(X)$. %\baigd{Readers don't know what is $\mathcal{F^\prime}$}
\end{definition}

\subsection{Workflow of \codename}
\label{sec:workflow}
 %We apply a two-layer architecture in \codename  by dividing the nodes into a local node layer which comprises of participating data owners, and an aggregation server which can be untrustworthy.
 %The dispensability of the multiplications and non-linear functions is achieved by encapsulating and distributing these operations to the nodes where the data resides on, instead of moving the data out of the nodes to the computation.
 %First, both of the raw data and model parameters are always kept in the local node layer, and every local node  %Every \highlight{party}\baigd{local node?}
 %is independently responsible for execute matrix multiplication on the plain data and parameter, and generates intermediate result.
 %These intermediate results will be protected by the additive secret sharing scheme~\cite{bogdanov2008sharemind} and only the \emph{sum} of these results will be sent to the aggregation server.
 %The server then performs the remaining computation which includes a series of multiplication operations and non-linear functions on the addition result, and sends its computation result back to the local nodes for them to update their parameters respectively and calculate the intermediate results for the next-round iteration.
 %As such, the multiplication and non-linear functions are all executed inside the nodes, and only homomorphic addition operation is required during the whole workflow for securely calculate the sum of the private intermediate results.

Figure \ref{fig:Gradient} illustrates the end-to-end workflow of the \codename, %. Now, we propose the privacy preserving collaborative learning framework for gradient descent optimization
which is divided into the following five steps.
%\vspace{-15pt}
\begin{figure}
	\includegraphics[width=\textwidth]{fig/Gradient.pdf}
	\centering
	\caption{The end-to-end workflow of the \codename.}
	\label{fig:Gradient}
\end{figure}

\textbf{Initialization}: At the beginning of learning task, each local node $S_l$ holds its own training data set $X^l$ %($l\in  \{1, ... , s\}$)
respectively, and randomly initializes the corresponding coefficient $W^l$.

\textbf{Step 1}: In each iteration of gradient descent, each local node computes linear combinations $X^lW^l$ locally. Note that, the information of $d_l$ is hidden by the matrix multiplication of $X^l \in \mathbb{R}^{m \times d_l}$ and $W^l \in \mathbb{R}^{d_l}$, and the result matrices $X^lW^l$ produced by all of local nodes have the same size of $\mathbb{R}^m$.

\textbf{Step 2}: Local nodes split  $X^lW^l$ into shares using $s$-out-of-$s$ \emph{additive secret sharing scheme} \cite{bogdanov2008sharemind}, such that  any set of at most $s-1$ shares gives no information about $X^lW^l$:
\begin{equation}
{\{(S_l, E_{X^lW^l})\}_{S_l \in S}} \leftarrow Shr(X^lW^l, S)
\end{equation}
, in which the sharing algorithm $Shr$ takes as input a secret $X^lW^l$ and a set
$S$ of local nodes, and produces a set of shares $E_{X^lW^l}$, each of which is
associated with a different $S_l \in S$.

% need to apply the addition operation on these $X^1W^1$,...,$X^sW^s$ to generate $XW = \sum\limits_{l=1}^{s} X^lW^l$. However, if we directly transfer $X^lW^l$ to the aggregation node to compute the sum, data information may be disclosed via the model updates. Therefore, in this step, we incorporate the $s$-out-of-$s$ Shamir's secret-sharing scheme  for the addition operation, which allows a user to split a secret $srt$ into $s$ shares, such that any $s$ shares can be used to reconstruct $srt$, but any set of at most $s-1$ shares gives no information about $srt$.
%The Shamir's secret-sharing, denoted by $Shr(srt^l, S) = {\{(S_l, E_{srt^l})\}_{S_l \in S}}$, takes as input a secret $srt^l$ and a set
%$S$ of local nodes, and produces a set of shares $E_{srt^l}$, each of which is
%associated with a different $S_l \in S$. In our framework, the concrete secret ($srt^l$) is set as $X^lW^l$.
%It keeps $X^lW^l$ secret, and it also keeps the whole protocol efficient, as computing the additions using Shamir's secret-sharing scheme is relatively computationally cost-efficient and does not require extra communication.
%We refer readers to \cite{shamir1979share,ben1988completeness} for more details of Shamir's secret-sharing scheme.
%By $srt^l = {X^lW^l}$, we assign the result of $X^lW^l$ to a secret  $srt^l$. $Shr(srt^l, S) = {\{(S_l, E_{srt^l})\}_{S_l \in S}}$ denotes secret sharing function that takes a secret $srt^l$, a set $S$ of local nodes as input, and produces a set of shares $E_{srt^l}$, each of which is associated with a different $S_l \in S$.

%the addition result $XW$
%But, if we directly transfer $X^lW^l$ to aggregation nodes to do the addition, the aggregation nodes then know each $X^lW^l$. This information combined with the $\Delta$ which they will compute later, ($\Delta$ contains the instruction of how to update the coefficients), makes it possible for aggregation nodes to identify the original training data in each single-point-analyze node.

%To solve the problem, we incorporate the Shamir's secret-sharing scheme \cite{shamir1979share} for the addition operation. It keeps $X^lW^l$ secret, and it also keeps the whole protocol efficient, as computing the additions using Shamir's secret-sharing scheme is relatively computationally cost-efficient and does not require extra communication.

\textbf{Step 3}: Reconstruct the homomorphic addition result $XW$ (equals $\sum\limits_{l=1}^{s} X^lW^l$) simply by adding the shares already have:
\begin{equation}
XW \leftarrow Rec(\{(S_l, E^l_{X^lW^l})\}_{S_l \in S})
\end{equation}

% additively shared value $$.

\textbf{Step 4}: Aggregation node computes $\Delta$, which as already noted in Section \ref{sec:gd}, is a function of $XW$, and sends $\Delta$ back to local nodes.

\textbf{Step 5}: Local nodes update the respective coefficient $W^l$ as:

\begin{equation}
W^l \leftarrow W^l - \alpha(\Delta X^l + \tau^l)
\end{equation}

Then these five steps are repeated for the next training iteration until convergence.
During the whole learning process, the local nodes keep their own training data $X^l$ and update the corresponding coefficient $W^l$ locally.

Note that, in our design, we let the aggregation server $Agg$ have the knowledge of $XW$ (i.e. the sum of $X^lW^l$).
We will show the privacy preservation as defined in Definition \ref{def:security} can be achieved with such knowledge and additional information learned from the training iteration  (Details given in Section \ref{sec:security}). %conditioned on a sufficiently large rank of training dataset.

%The framework can also be used to securely make predictions as well as test the accuracy of the current model. After the aggregation node computes the addition result $XW$, it only needs to compute $\sigma(XW)$, since the prediction is simply to compute $\sigma(XW)$, and the accuracy is simply an aggregated result of the predictions on the testing data.

%Later, we prove that, the joint view of any subset of local nodes, additionally combine with the aggregation node learn nothing more than their own inputs, besides what can be inferred from the output of the computation. More details regarding the party knowledge of our framework will be discussed in Section \ref{sec:PartyKnowledge}.






==> chapters/design1.tex <==
\section{Design of \codename}
\label{sec:design}
%In this section, we present the privacy preserving collaborative framework for machine learning algorithms using gradient descent for optimization.


\subsection{Threat Model}
\label{sec:threat}
The involved parties in \codename are a set of local nodes (i.e., data owners) $S_1, ..., S_s$ and an aggregation node  $Agg$. %\highlight{server} \baigd{I would suggest node as server sounds like centralized stuff. Be consistent throughout the whole paper}
<<<<<<< HEAD
Each local node holds part of \highlight{features} \baigd{this matches the vertical concatenation, so you can justify it here. Refer to KDD paper, which mentions this} of the training samples, denoted by $X^l$ $(l \in \{1,...,s\})$, and the corresponding local model $W^l$ $(l \in \{1,...,s\})$ trained on $X^l$.
Each $X^l \in \mathbb{R}^{m \times d_l}$ is a $m \times d_l$ matrix representing $m$ training samples with $d_l$ features, and $W^l \in \mathbb{R}^{d_l}$ is a \baigd{$d_1 \times 1$?} vector of coefficients. 
In \codename, $m$  is public and known by every party, and $d_l$  is private and only known by the corresponding data owner $S_l$. 
We use $X$ to denote the \highlight{vertical concatenation} \baigd{refer to ``features'' above. in addition, reviewer may ask whether it is realistic to assume local datasets can be vertically concatenated - this requires everyone has the same $m$, and it is semantically correct to concatenate all the i-th rows. Any literature to support?}  of the local training datasets $X^1, ..., X^s$.
Then we know that $X$ is a $m \times n$ matrix  %\baigd{This means the dataset are cut vertically. Is this realistic?} \yanjun{I thought it is realistic, for example, health institutions in a certain area may share a large number of common patients, say a patient did a blood test in a pathology lab, might also have a CT scan record in another radiology center, or might occasionally visit hospital emergency departments. Such collaboration can improve the predictive power by leveraging additional features from other domain or parties.}
%\baigd{\\ If so, is this common in the literature? If not, the applicability and usability needs to be made clear and discussed \\}
where $n = \sum_{l=1}^{s}d_l$ (i.e., the total number of features in $X$). 
Since $d_l$  is private, $n$ is unknown to every individual local node unless all of them join their views.
=======
Each local node holds part of features of the training samples, denoted by $X^l$ $(l \in \{1,...,s\})$, and the corresponding local model $W^l$ $(l \in \{1,...,s\})$ trained on $X^l$.
Each $X^l$ is a $m \times d_l$ matrix representing $m$ training samples with $d_l$ features.
In \codename, $m$  is public and known by every party, and $d_l$  is private and only known by the corresponding data owner $S_l$.
Let $X$ be a $m \times n$ matrix to denote the vertical concatenation %\highlight{vertical concatenation} %\baigd{This means the dataset are cut vertically. Is this realistic?} \yanjun{I thought it is realistic, for example, health institutions in a certain area may share a large number of common patients, say a patient did a blood test in a pathology lab, might also have a CT scan record in another radiology center, or might occasionally visit hospital emergency departments. Such collaboration can improve the predictive power by leveraging additional features from other domain or parties.} 
%\baigd{\\ If so, is this common in the literature? If not, the applicability and usability needs to be made clear and discussed \\} 
of the local training datasets $X^1, ..., X^s$, where $n = \sum_{l=1}^{s}d_l$.
Since $d_l$  is private, $n$ (i.e., the number of overall features in $X$) is unknown unless all of local nodes join their views.
>>>>>>> d8595e01e228ccd7228464d1b45071f9d8f1cfa9

\codename targets to defend against an honest-but-curious adversary $\mathcal{A}$, who follows the collaboration protocols and training procedures, but aims to obtain the datasets of other local nodes~(i.e., $X^l$) and/or the model parameters trained out of them~(i.e., $W^l$).
The adversary may control $Agg$, and $t$ out of $s$ local nodes. Here, we conservatively assume $t < s-1$, which implies that at least two local nodes need to be out of the adversary's control, as $s-1$ comprised local nodes who has the sum of their shares, colluding with $Agg$ who has the sum of all shares, will be able to obtain the share of the remaining node by a simple subtraction%\replace{as the local nodes who collude with $Agg$ will have the knowledge of the \emph{sum} of the intermediate results produced by other honest nodes}{as $s-1$ comprised local nodes who has the sum of their shares, colluding with $Agg$ who has the sum of all shares, will be able to obtain the share of the remaining node by a simple subtraction}
~(detailed in Section \ref{sec:security}).
%Therefore, to achieve the privacy preservation, we need at least $2$ honest local nodes in \codename (Detailed in Section \ref{sec:security}).


\subsection{Definitions of Privacy Preservation and Correctness}
Keeping local data/model private and providing functional correctness are the main properties \codename aims to achieve. Below we present the definition of these two properties.
\begin{definition}
	\label{def:security}
	\textbf{($\varepsilon$-privacy)}
A mechanism preserves $\varepsilon$-privacy if the probability for a probabilistic polynomial-time (PPT) adversary to derive $X^l$ or $W^l$ based on its knowledge is $\leq \varepsilon$.
\end{definition}

\begin{definition}
	\label{def:correct}
	\textbf{(Correctness)}
	Given a function $\mathcal{F}$ that takes as input a training dataset $X$, and its distributed version $\mathcal{F^\prime}$ that takes as inputs $X$'s vertical partitions $X^1, ..., X^s$, we say
$\mathcal{F^\prime}$ is correct if $\mathcal{F^\prime}(\{(S_l, X^l), Agg\}_{S_l \in S})=\mathcal{F}(X)$.
\end{definition}

\subsection{Workflow of \codename}
\label{sec:workflow}
 %We apply a two-layer architecture in \codename  by dividing the nodes into a local node layer which comprises of participating data owners, and an aggregation server which can be untrustworthy.
 %The dispensability of the multiplications and non-linear functions is achieved by encapsulating and distributing these operations to the nodes where the data resides on, instead of moving the data out of the nodes to the computation.
 %First, both of the raw data and model parameters are always kept in the local node layer, and every local node  %Every \highlight{party}\baigd{local node?}
 %is independently responsible for execute matrix multiplication on the plain data and parameter, and generates intermediate result.
 %These intermediate results will be protected by the additive secret sharing scheme~\cite{bogdanov2008sharemind} and only the \emph{sum} of these results will be sent to the aggregation server.
 %The server then performs the remaining computation which includes a series of multiplication operations and non-linear functions on the addition result, and sends its computation result back to the local nodes for them to update their parameters respectively and calculate the intermediate results for the next-round iteration.
 %As such, the multiplication and non-linear functions are all executed inside the nodes, and only homomorphic addition operation is required during the whole workflow for securely calculate the sum of the private intermediate results.

Figure \ref{fig:Gradient} illustrates the end-to-end workflow of \codename, %. Now, we propose the privacy preserving collaborative learning framework for gradient descent optimization
which is divided into the following steps.
%\vspace{-15pt}
\begin{figure}
	\includegraphics[width=\textwidth]{fig/Gradient.pdf}
	\centering
	\caption{The end-to-end workflow of the \codename} %\baigd{it is not clear who executes 2 and 3. the rectangle may be confusing, as it doesn't belong to local nodes or agg}
%\baigd{one thing unclear to me: the scheme must be executed by the participant, but how is this done is not mentioned at all. See my comments for step 3 below}
	\label{fig:Gradient}
\end{figure}

\textbf{Initialization}: Each local node $S_l$ holds its own training dataset $X^l \in \mathbb{R}^{m \times d_l}$, and randomly initializes its coefficient \baigd{coefficient vector? coefficient sounds like one single } $W^l \in \mathbb{R}^{d_l}$.

\textbf{Step 1}: In each iteration of gradient descent, each $S_l$ multiplies $X^l$ by $W^l$ locally,   resulting in a $X^lW^l \in \mathbb{R}^m$. 
%computes matrix multiplication %\highlight{linear combinations} \baigd{this implies $W^l$ is a vector. then I feel the link of $W$ and $W^l$ should be mentioned somewhere?}
%$X^lW^l \in \mathbb{R}^m$ locally. 
The information of $d_l$, the number of features in $X^l$, is removed by such a matrix multiplication.

\textbf{Step 2}: Each $S_l$ executes the sharing algorithm $Shr$ to split $X^lW^l$ into shares using the \emph{additive secret sharing scheme}.
\begin{equation}
{\{(S_i, E^i_{X^lW^l})\}_{S_i \in S}} \leftarrow Shr(X^lW^l, S),
\end{equation}
in which $Shr$  takes as input a secret $X^lW^l$ and a set
$S$ of local nodes, and produces a set of shares $E^i_{X^lW^l} (i \in \{1,...,s\})$, each of which is distributed to a different $S_i \in S$.  Then, each  $S_l$ calculates the sum of all shares it receives, and gets $E^l = \sum_{j = 1}^s E_{X^jW^j}^l$.
%\baigd{mathematically wrong here: the $l$ in $X^lW^l$ and the $l$ in $E^l$ are different.}
%\baigd{what you want is ``for each $S_i \in S$, it produces the share $E^i_{X^lW^l}$''}
%\baigd{check this in equation 4 and 5 as well!}

% need to apply the addition operation on these $X^1W^1$,...,$X^sW^s$ to generate $XW = \sum\limits_{l=1}^{s} X^lW^l$. However, if we directly transfer $X^lW^l$ to the aggregation node to compute the sum, data information may be disclosed via the model updates. Therefore, in this step, we incorporate the $s$-out-of-$s$ Shamir's secret-sharing scheme  for the addition operation, which allows a user to split a secret $srt$ into $s$ shares, such that any $s$ shares can be used to reconstruct $srt$, but any set of at most $s-1$ shares gives no information about $srt$.
%The Shamir's secret-sharing, denoted by $Shr(srt^l, S) = {\{(S_l, E_{srt^l})\}_{S_l \in S}}$, takes as input a secret $srt^l$ and a set
%$S$ of local nodes, and produces a set of shares $E_{srt^l}$, each of which is
%associated with a different $S_l \in S$. In our framework, the concrete secret ($srt^l$) is set as $X^lW^l$.
%It keeps $X^lW^l$ secret, and it also keeps the whole protocol efficient, as computing the additions using Shamir's secret-sharing scheme is relatively computationally cost-efficient and does not require extra communication.
%We refer readers to \cite{shamir1979share,ben1988completeness} for more details of Shamir's secret-sharing scheme.
%By $srt^l = {X^lW^l}$, we assign the result of $X^lW^l$ to a secret  $srt^l$. $Shr(srt^l, S) = {\{(S_l, E_{srt^l})\}_{S_l \in S}}$ denotes secret sharing function that takes a secret $srt^l$, a set $S$ of local nodes as input, and produces a set of shares $E_{srt^l}$, each of which is associated with a different $S_l \in S$.

%the addition result $XW$
%But, if we directly transfer $X^lW^l$ to aggregation nodes to do the addition, the aggregation nodes then know each $X^lW^l$. This information combined with the $\Delta$ which they will compute later, ($\Delta$ contains the instruction of how to update the coefficients), makes it possible for aggregation nodes to identify the original training data in each single-point-analyze node.

%To solve the problem, we incorporate the Shamir's secret-sharing scheme \cite{shamir1979share} for the addition operation. It keeps $X^lW^l$ secret, and it also keeps the whole protocol efficient, as computing the additions using Shamir's secret-sharing scheme is relatively computationally cost-efficient and does not require extra communication.

\textbf{Step 3}: %\baigd{Who}
%\baigd{there should be at least one sentence to describe how $E^l_{X^lW^l}$ reach $Agg$ before it can  }
$Agg$ collects all $E^l$ from local nodes, and reconstructs the homomorphic addition result $XW$ (equals $\sum\limits_{l=1}^{s} X^lW^l$) by adding $E^l$ together %simply by adding the shares \highlight{already have:} \baigd{what does this mean?}
\begin{equation}
XW \leftarrow Rec(\{(S_l, E^l)\}_{S_l \in S})
\end{equation}

\baigd{Does Rec make any sense here? why not simply: }
\begin{equation}
XW \leftarrow \sum_{l = 1}^s E^l = \sum_{l = 1}^s \sum_{j = 1}^s E_{X^jW^j}^l = \sum_{j = 1}^s \sum_{l = 1}^s E_{X^jW^j}^l = \sum_{j = 1}^s X^jW^j
\end{equation}

% additively shared value $$.

\textbf{Step 4}: %\highlight{Aggregation node} \baigd{make it consistent: Aggregation node, aggregation server, or $Agg$}
$Agg$ computes $\Delta = \frac{\partial{J}}{\partial{\sigma}}\frac{\partial{\sigma}}{\partial{XW}}$ (\emph{c.f.}, Equation \ref{equ:chain}), %\highlight{which as already noted in Section \ref{sec:gd}, is a function of $XW$,} \baigd{this sentence is not informative at all. it may irritate readers. either copy $\Delta = \frac{\partial{J}}{\partial{\sigma}}\frac{\partial{\sigma}}{\partial{XW}}$ here, or refer to equation 2.}
and sends $\Delta$ back to local nodes.

\textbf{Step 5}: With the received $\Delta$, each $S_l$ updates its local \highlight{coefficient matrix} \baigd{when you rename it at one place, make sure propagate to every occurance} %\baigd{vector}
$W^l$ as:

\begin{equation}
W^l \leftarrow W^l - \alpha(\Delta X^l + \tau^l)
\end{equation}

\textbf{Step 1-5} are repeated for the next training iteration until convergence.

During the whole learning process, the local nodes keep their own training data $X^l$ and update the corresponding coefficient $W^l$ locally.
\highlight{The intermediate results $X^lW^l$ generated by local nodes are protected by the additive secret sharing scheme, and $XW$ (i.e., the sum of $X^lW^l$) will be sent to $Agg$.}
\baigd{rewrite this sentence: from the perspective of a local node, ...; from the perspective of $Agg$, ...}



%\baigd{revise the following paragraph to include two ideas: \\
%1) local nodes: privacy leakage to local nodes is prevented by the additive secret sharing scheme \\
%2) aggregation server: ... \\ }
%In our design, the \highlight{aggregation server $Agg$} \baigd{if the full name has to be repeated at every occurrence, the abbreviation doesn't have to be defined} has the knowledge of $XW$ (i.e., the sum of $X^lW^l$).
%We will show the privacy preservation as defined in Definition \ref{def:security} can be achieved with such knowledge and additional information learned from the training iteration  (Details given in Section \ref{sec:security}). %conditioned on a sufficiently large rank of training dataset.

%The framework can also be used to securely make predictions as well as test the accuracy of the current model. After the aggregation node computes the addition result $XW$, it only needs to compute $\sigma(XW)$, since the prediction is simply to compute $\sigma(XW)$, and the accuracy is simply an aggregated result of the predictions on the testing data.

%Later, we prove that, the joint view of any subset of local nodes, additionally combine with the aggregation node learn nothing more than their own inputs, besides what can be inferred from the output of the computation. More details regarding the party knowledge of our framework will be discussed in Section \ref{sec:PartyKnowledge}.






==> chapters/intro.tex <==
\section{Introduction}

Collaborative machine learning is an emerging technique that allows two or more data owners, each with its own training dataset, to construct a joint model. 
Preserving privacy during collaborative learning requires protecting not only the data, but also the locally trained model, since a direct release of trained models carries the risk of disclosing private information~\cite{melis2019exploiting}. 
For example, a model-inversion attack was demonstrated in~\cite{fredrikson2015model} to extract training data only with access to the trained model.
%For example, a classifier model may reveal the features that characterize a given class or help construct data points that belong to this class. 
In addition, in the cases where the model itself represents intellectual property, it is a necessary requirement that the model and its parameters be confidential~\cite{papernot2016towards}, e.g., financial market systems.

The existing techniques of preserving privacy include differentially private machine learning frameworks and cryptographic solutions. %, such as homomorphic encryption (HE)~\cite{gentry2009fully} and secure multiparty computation (MPC)~\cite{yao1986generate, goldreich2019play}. 
The former usually employ noise mechanisms for privacy preservation and thus introduce a cost of loss in model accuracy~\cite{abadi2016deep, song2013stochastic, shokri2015privacy, zheng2019bdpl, dwork2014algorithmic, hu2019fdml}. 
To retain the original accuracy of the training model in this work, we therefore turn to the cryptographic line of studies which are able to compute identical results from the cyphertext as from the plaintext. 
However, most existing cryptographic machine learning frameworks rely on heavy cryptographic techniques such as (fully) homomorphic encryption (HE)~\cite{gentry2009fully, chen2018privacy, marc2019privacy, sharma2019confidential}  and generic secure multiparty computation (MPC)~\cite{yao1986generate, goldreich2019play, gascon2017privacy, gascon2016secure, liu2017oblivious, mohassel2017secureml, bonawitz2017practical}, which are known to be limited by significant overhead.
Specifically, the overhead introduced by the  schemes above mainly lies in the cryptographic implementation of multiplication operations and non-linear functions (and we note such operations are intensively used in machine learning algorithms), whereas most cryptographic schemes are much more communicationally and computationally efficient in \emph{addition operation}.

%The existing techniques of preserving privacy include differentially private machine learning frameworks~\cite{abadi2016deep, song2013stochastic, shokri2015privacy, zheng2019bdpl, dwork2014algorithmic, hu2019fdml} and cryptographic solutions, such as homomorphic encryption (HE)~\cite{gentry2009fully, chen2018privacy, marc2019privacy, sharma2019confidential} and secure multiparty computation (MPC)~\cite{gascon2017privacy, gascon2016secure, liu2017oblivious, mohassel2017secureml, zheng2019towards, bonawitz2017practical}. 
%While most existing differentially private mechanisms achieve privacy preservation at a cost of loss in model accuracy, the cryptographic solutions, on the other hand, are able to compute identical results from the cyphertext as from the plaintext, but are known to be limited by significant overhead.
%In particular, most HE/MPC schemes are communicationally and computationally efficient in  \emph{addition operation}, however, costly in multiplication and non-linear functions, resulting in a less practicability for machine learning algorithms in which multiplication and non-linear functions are very commonly used. 

In this work, we propose the \codename, a lightweight cryptographic framework based on the \emph{additive secret sharing scheme}~\cite{bogdanov2008sharemind}, tailored for privacy-preserving collaborative machine learning. 
To achieve the practicability, we carefully designed our workflow to deliberately avoid costly cryptographic implementations of multiplication and non-linear operations, and the \emph{additive secret sharing scheme} is employed for homomorphic \emph{addition operation} only, which is a distinct advantage of \codename over prior art for privacy-preserving machine learning deployment.
Note that, our design is based on the observation that training datasets nowadays are usually of large size.   
In \codename, the security is guaranteed conditioned on a sufficiently large rank of training dataset.

In a nutshell, we apply a two-layer architecture in our approach by dividing the nodes into a local node layer which comprises of data owners who participate in the collaborative learning, and an unnecessarily trustworthy aggregation server layer.
Both original data and model parameters are kept in the local node layer to ensure confidentiality. 
During each iteration of the training process, each local node performs computation on the data and the parameters, and generates intermediate results. 
These intermediate results will then be summed up through \emph{additive secret sharing scheme} to the aggregation server. 
The server then performs the remaining computation of the current iteration and sends the computation results back to the local nodes for them to update their parameters respectively and calculate the intermediate results for the next-round iteration. 
This process repeats until the optimization converges.
We prove that, only with the sum of these intermediate results and additional knowledge learned from the training iterations, the probability for corrupted parties of revealing either the original data or the trained parameters from other honest parties is negligible, provided that the composite training dataset is of a sufficiently large rank.


Notably, \codename induces none sacrifice to the accuracy of models and also supports a wide range of machine learning algorithms---we prove that it preserves the correctness of any algorithms that use gradient descent for optimization, including but not limited to linear regression, logistic regression, a variety of neural networks, and etc.

 
 
\subsection{Contributions}
 In general, our contributions can be summarized as follows.
\begin{itemize}
	\item \textbf{A Novel Privacy-preserving Collaborative Framework.} 
	We propose a novel framework \codename for privacy-preserving collaborative learning while enabling a wide range of machine learning algorithms and achieving high computation efficiency. 
	In \codename, not only original data, but also trained parameters are kept locally to ensure both the data and the trained model be confidential.

	\item \textbf{Provable Security and Correctness Guarantee.} 
	We prove the security of \codename, demonstrating a negligible probability for corrupted parties of revealing either the original data or the trained parameters from other honest parties. %, conditioned on a sufficiently large rank of training dataset.  
	We also ensure the learning results to be exactly same in \codename as it is in the traditional non-distributed framework to guarantee the correctness. 

	\item \textbf{Experimental Evaluations.} We run experiments on real datasets showing the significant improvement of efficiency of \codename compared with the state-of-the-art MPC and HE algorithms. 
	For example, \codename  achieves around $22.5$ minutes for a two-hidden-layer neural network to process all samples in the MNIST dataset~\cite{lecun-mnisthandwrittendigit-2010}, while it takes more than $81$ hours with a state-of-the-art MPC protocol SecureML~\cite{mohassel2017secureml}.
\end{itemize}

\subsection{Organization}
The rest of the paper is organized as follows. We briefly introduce necessary backgrounds of gradient descent and additive secret sharing scheme in Section \ref{sec:background}, and we present our design of \codename in Section \ref{sec:design}. We then prove the security of \codename in Section \ref{sec:security}, and demonstrate its correctness and provide a case study of recurrent neural network  in Section \ref{sec:corr&case}.  The efficiency performance are illustrated in Section \ref{sec:performance}. Section \ref{sec:related} reviews related works, and some concluding remarks are given in Section \ref{sec:conclusion}.

==> chapters/intro1.tex <==
\section{Introduction}

The performance of machine learning largely relies on the availability of data.
To take advantage of massive data owned by multiple entities,
the collaborative machine learning has been proposed to enable two or more data owners to construct a joint model.
In practice, however, this incurs privacy concerns.
The data owners usually require the raw data to be confined locally, and they may also demand the protection of the locally trained models, since a direct release of trained models carries the risk of disclosing private information~\cite{melis2019exploiting}.
For example, a model-inversion attack was demonstrated in~\cite{fredrikson2015model} to extract training data only with access to the trained models.
%For example, a classifier model may reveal the features that characterize a given class or help construct data points that belong to this class.
In addition, in the cases where the model itself represents intellectual property, e.g., in financial market systems, it is an essential requirement that the model and its parameters are kept confidential~\cite{papernot2016towards}.

%\baigd{I don't recommend to take HE and MPC as the main competitors. They are both too distant from this work. As a reference, you may refer to the KDD paper (FDML). Look at its related work section. The mentioned distributed machine learning, model parallelism, etc., are your competitors, or at least research context of this work. You need to justify how your work advances them, not HE/MPC. Actually, you will find most of them are advances of HE and MPC. }
%\baigd{The reviewers will NOT actively look for the novelty from your technical sections. This is not their obligation. That is why PAKDD reviewers complained our novelty. Instead, they will be passively told by your paper and judge the validity of your statements. If you position your work as an advance of HE/MPC, rather than the research context in privacy-preserving learning, or distributed learning, the reviewers will definitely attack the novelty again. }
%The existing techniques of preserving privacy include differentially private machine learning frameworks~\cite{abadi2016deep, song2013stochastic, shokri2015privacy, zheng2019bdpl, dwork2014algorithmic} and cryptographic solutions, such as homomorphic encryption (HE)~\cite{gentry2009fully, chen2018privacy, marc2019privacy, sharma2019confidential} and secure multiparty computation (MPC)~\cite{gascon2017privacy, gascon2016secure, liu2017oblivious, mohassel2017secureml, zheng2019towards, bonawitz2017practical}.
%While most existing differentially private mechanisms achieve privacy preservation at a cost of loss in model accuracy, the cryptographic solutions, on the other hand, are able to compute identical results from the cyphertext as from the plaintext, but are known to be limited by significant overhead.
%In particular, most HE/MPC schemes are communicationally and computationally efficient in  \emph{addition operation}, however, costly in multiplication and non-linear functions, resulting in a less practicability for machine learning algorithms in which multiplication and non-linear functions are very commonly used.

The existing techniques of preserving privacy in collaborative learning include differentially private mechanisms and cryptographic solutions. %, such as homomorphic encryption (HE)~\cite{gentry2009fully} and secure multiparty computation (MPC)~\cite{yao1986generate, goldreich2019play}.
The former are often on an ad-hoc basis~\cite{zheng2019bdpl, hagestedt2019mbeacon}, and those for general purpose usually entail adding noise on the training data, causing loss in model accuracy~\cite{abadi2016deep, song2013stochastic, shokri2015privacy , dwork2014algorithmic, hu2019fdml}.
Therefore, the cryptographic solutions, which are able to yield identical models as from training on plaintext data, has become appealing.
Nevertheless, most existing cryptographic machine learning frameworks rely on heavy cryptographic techniques such as (fully) homomorphic encryption (HE)~\cite{ chen2018privacy, marc2019privacy, sharma2019confidential}  and generic secure multiparty computation (MPC)~\cite{ gascon2017privacy, gascon2016secure, liu2017oblivious, mohassel2017secureml, bonawitz2017practical}, which are known to be limited by significant overhead.


%most cryptographic schemes are communicationally and computationally efficient in \emph{addition operation}, however, much more costly in cryptographic implementations of multiplication operation and non-linear functions (and we note such operation and functions are intensively used in machine learning algorithms) and thus results in the less practicability.

%

In this work, we aim to enhance the practicability of the cryptographic solutions by developing a lightweight framework named \codename.
\codename is motivated by addressing the problem that the overhead of cryptographic algorithms
mainly lies in the heavy implementations of \emph{multiplication operation} and \emph{non-linear functions} that are far more costly in computation/communication than that of \emph{addition operation} \cite{gentry2009fully,albrecht2018homomorphic,yao1986generate, goldreich2019play}. %\baigd{any citation or study to support this statement?}
We design a novel workflow of collaborative learning %, \highlight{in which the multiplication and non-linear operations are replaced with the homomorphic addition operation provided by the tailored \emph{additive secret sharing scheme}~\cite{bogdanov2008sharemind}}\baigd{check this}.
in which the cryptographic implementations of the multiplication and non-linear operations are dispensable. 
%, and the \highlight{privacy preservation is guaranteed with the homomorphic addition operation provided by \emph{additive secret sharing scheme}~\cite{bogdanov2008sharemind}}. \baigd{1) seems vague to use just one sentence to explain how privacy---the main contribution---is solved, 2) a bit sudden to talk about privacy preservation here while you are talking about the two operations. Readers are expecting to see how existing learning still work after dispensing multiplication.}
%The dispensability of the multiplications is achieved \highlight{by the preservation of data locality in \codename.} \baigd{``by something'' implies ``something'' is a mechanism, but data locality is the goal, is it?} 

We apply a two-layer architecture in \codename  by dividing the nodes into a local node layer which comprises of data owners, and aggregation server layer which can be untrustworthy. 
The dispensability of the multiplications and non-linear functions is achieved by encapsulating and distributing these operations to the nodes where the data resides on, instead of moving the data out of the nodes to the computation. 
First, the raw data and model parameters are always kept in the local node layer, and every local node  %Every \highlight{party}\baigd{local node?} 
is independently responsible for execute multiplication on the data and the parameter, and generates intermediate result. 
These intermediate results will be protected by the additive secret sharing scheme~\cite{bogdanov2008sharemind} and only the \emph{sum} of these results will be sent to the aggregation server. 
The server then performs the remaining computation, which is an encapsulation of a series of multiplication operations and non-linear functions, and sends the computation results back to the local nodes for them to update their parameters respectively and calculate the intermediate results for the next-round iteration. 
As such, the multiplication and non-linear functions are all executed inside the nodes, and only homomorphic addition operation is required during the whole workflow for securely calculate the sum of the private intermediate results. 

% be moved around amongst the involved parties to achieve the final joint learning model.  %and with .
%\baigd{Weave the workflow with the statements above: } Below we summarize our workflow in a nutshell. During each iteration of the training process, each local node first performs matrix multiplication on the data and the parameters locally, and generates the intermediate results.
%These intermediate results will then be summed up through the additive secret sharing scheme to the aggregation server.
%The server then performs the remaining computation of the current iteration, which is an encapsulation of a series of multiplication operations and non-linear functions, and sends the computation results back to the local nodes for them to update their parameters respectively and calculate the intermediate results for the next-round iteration.
%This process repeats until the optimization converges.
%As such, by encapsulating and distributing multiplication and non-linear operations to different layer of participants, we can remove the cryptographic implementations of these operations

\codename is designed to preserve privacy in a way that the \emph{honest-but-curious} participants, who have access to the sum of the intermediate results produced by local nodes and additional knowledge learned from the training iterations, are unlikely~(i.e., with a negligible probability) to reveal the raw data or the local model parameters of other participants.
As a side effect of removing the cryptographic implementations of multiplications, the adversary obtains the \emph{party knowledge} from training iteration~(detailed in Section~\ref{sec:party}). %of some unencrypted intermediate results.
We prove that with a sufficient rank of the training dataset ($\geq$ 32 that is common in real-world datasets), \codename achieves the desired privacy preservation.

Notably, \codename introduces none sacrifice to the accuracy of models and also supports a wide range of machine learning algorithms. Intuitively, our solution makes use of chain rules in calculus applied in gradient descent optimization, and ensures that the computation executed by the aggregation node is only associated with the \emph{sum} of the intermediate results generated by local nodes.
We prove such correctness guarantee of any algorithms that use gradient descent for optimization, including but not limited to linear regression, logistic regression, and a variety of neural networks.

\paragraph{Contributions}
 In general, our contributions can be summarized as follows.
\begin{itemize}
	\item \textbf{A Novel Privacy-preserving Collaborative Framework.}
	We propose a novel framework \codename for privacy preserving collaborative learning while enabling a wide range of machine learning algorithms and achieving high computation efficiency.
	In \codename, not only original data, but also trained parameters are kept locally to ensure both the data and the trained model be confidential.

	\item \textbf{Provable Privacy Preservation and Correctness Guarantee.}
	We prove the privacy preservation %\highlight{security} \baigd{Is this security or privacy}
	of \codename, demonstrating a negligible probability for corrupted parties of revealing either the original data or the trained parameters from other honest parties. %, conditioned on a sufficiently large rank of training dataset.
	We also ensure the learning results to be exactly same in \codename as it is in the traditional non-distributed framework to guarantee the correctness.

	\item \textbf{Experimental Evaluations.} We run experiments on real datasets showing the significant improvement of efficiency of \codename compared with the state-of-the-art MPC and HE algorithms.
	For example, \codename  achieves around $22.5$ minutes for a two-hidden-layer neural network to process all samples in the MNIST dataset~\cite{lecun-mnisthandwrittendigit-2010}, while it takes more than $81$ hours with a state-of-the-art MPC protocol SecureML~\cite{mohassel2017secureml}.
\end{itemize}

\paragraph{Organization}
The rest of the paper is organized as follows. We briefly introduce necessary backgrounds of gradient descent and additive secret sharing scheme in Section \ref{sec:background}, and we present our design of \codename in Section \ref{sec:design}. We then prove the privacy preservation of \codename in Section \ref{sec:security}, and demonstrate its correctness and provide a case study of recurrent neural network in Section \ref{sec:corr&case}.  The efficiency performance are illustrated in Section \ref{sec:performance}. Section \ref{sec:related} reviews related works, and some concluding remarks are given in Section \ref{sec:conclusion}.


==> chapters/intro2.tex <==
\section{Introduction}

The performance of machine learning largely relies on the availability of data.
To take advantage of massive data owned by multiple entities,
the collaborative machine learning has been proposed to enable two or more data owners to construct a joint model.
\add{To address the privacy concerns arising from the collaboration,}
\add{many studies~\cite{chen2018privacy, wang2019scalable, gascon2017privacy, zhang2019pefl} have managed to provide data locality by distributing learning algorithms onto data owners such that the data can be confined within the owners, and using an aggregation server to come up with the final model.}
%\baigd{distributing the learning algorithm onto data owners}
Despite this, such solutions still entail sharing and synchronizing on the locally trained models \baigd{is locally trained models equivalent to the local model parameters?} \yanjun{yes, they are equivalent} and intermediate results which may imply privacy-sensitive information~\cite{melis2019exploiting}.
For example, a model-inversion attack was demonstrated in~\cite{fredrikson2015model} to extract training data only with access to the trained models.
In addition, in the cases where the model itself represents intellectual property, e.g., in financial market systems, it is an essential requirement that the model and its parameters are kept confidential~\cite{papernot2016towards}.

To enable the privacy-preserving sharing of the local models and intermediate results, two categories of techniques, i.e. differentially private mechanisms and cryptographic solutions, can be employed.
The former are often on an ad-hoc basis~\cite{zheng2019bdpl, hagestedt2019mbeacon}, and those for general purpose usually entail adding noise on the training data, causing loss in accuracy of the final models~\cite{abadi2016deep, song2013stochastic, shokri2015privacy , dwork2014algorithmic, hu2019fdml}.
Therefore, the cryptographic solutions, which are able to yield identical models as from training on plaintext data, has become appealing.
Nevertheless, most existing cryptographic machine learning frameworks rely on heavy cryptographic techniques such as (fully) homomorphic encryption (HE)~\cite{ chen2018privacy, marc2019privacy, sharma2019confidential}  and generic secure multiparty computation (MPC)~\cite{ gascon2017privacy, gascon2016secure, liu2017oblivious, mohassel2017secureml, bonawitz2017practical} \add{based on garbled circuits \cite{yao1986generate} and GMW protocol \cite{goldreich2019play}} \yanjun{garbled circuits and GMW protocol are specific protocols commonly used in MPC}, which are known to be limited by significant overhead.


%most cryptographic schemes are communicationally and computationally efficient in \emph{addition operation}, however, much more costly in cryptographic implementations of multiplication operation and non-linear functions (and we note such operation and functions are intensively used in machine learning algorithms) and thus results in the less practicability.

%

In this work, we aim to enhance the practicability of the cryptographic solutions \add{in a multiparty computation environment} by developing a lightweight framework named \codename.
\codename is motivated by addressing the problem that the overhead of cryptographic algorithms
mainly lies in the heavy implementations of \emph{multiplication operation} and \emph{non-linear functions} that are far more costly in computation/communication than that of \emph{addition operation} \cite{gentry2009fully,albrecht2018homomorphic,yao1986generate, goldreich2019play}. %\baigd{any citation or study to support this statement?}
The main idea is to design a novel workflow of collaborative learning %, \highlight{in which the multiplication and non-linear operations are replaced with the homomorphic addition operation provided by the tailored \emph{additive secret sharing scheme}~\cite{bogdanov2008sharemind}}\baigd{check this}.
\replace{in which the cryptographic implementations of the multiplication and non-linear operations are dispensable.} {in which the implementations of the multiplication and non-linear operations on encrypted data are dispensable, and only homomorphic addition operation, provided by \emph{additive secret sharing scheme}~\cite{bogdanov2008sharemind}, is required during the whole workflow.} \add{In a nutshell, we apply a two-layer architecture in \codename  by dividing the nodes into a local node layer which comprises of participating data owners, and an aggregation server which can be untrustworthy. Both of the raw data and model parameters are always kept in the local node layer, and the computation executed by the aggregation node is only associated with the \emph{sum} of the intermediate results generated by local nodes~(detailed in Section~\ref{sec:workflow}).
As such, we achieve significant  cost savings compared with state-of-art garbled circuits and GMW based MPC protocol.}

%, and the \highlight{privacy preservation is guaranteed with the homomorphic addition operation provided by \emph{additive secret sharing scheme}~\cite{bogdanov2008sharemind}}. \baigd{1) seems vague to use just one sentence to explain how privacy---the main contribution---is solved, 2) a bit sudden to talk about privacy preservation here while you are talking about the two operations. Readers are expecting to see how existing learning still work after dispensing multiplication.}
%The dispensability of the multiplications is achieved \highlight{by the preservation of data locality in \codename.} \baigd{``by something'' implies ``something'' is a mechanism, but data locality is the goal, is it?}

%We apply a two-layer architecture in \codename  by dividing the nodes into a local node layer which comprises of participating data owners, and an aggregation server which can be untrustworthy.
%The dispensability of the multiplications and non-linear functions is achieved by encapsulating and distributing these operations to the nodes where the data resides on, instead of moving the data out of the nodes to the computation.
%First, both of the raw data and model parameters are always kept in the local node layer, and every local node  %Every \highlight{party}\baigd{local node?}
%is independently responsible for execute matrix multiplication on the plain data and parameter, and generates intermediate result.
%These intermediate results will be protected by the additive secret sharing scheme~\cite{bogdanov2008sharemind} and only the \emph{sum} of these results will be sent to the aggregation server.
%The server then performs the remaining computation which includes a series of multiplication operations and non-linear functions on the addition result, and sends its computation result back to the local nodes for them to update their parameters respectively and calculate the intermediate results for the next-round iteration.
%As such, the multiplication and non-linear functions are all executed inside the nodes, and only homomorphic addition operation is required during the whole workflow for securely calculate the sum of the private intermediate results.


% be moved around amongst the involved parties to achieve the final joint learning model.  %and with .
%\baigd{Weave the workflow with the statements above: } Below we summarize our workflow in a nutshell. During each iteration of the training process, each local node first performs matrix multiplication on the data and the parameters locally, and generates the intermediate results.
%These intermediate results will then be summed up through the additive secret sharing scheme to the aggregation server.
%The server then performs the remaining computation of the current iteration, which is an encapsulation of a series of multiplication operations and non-linear functions, and sends the computation results back to the local nodes for them to update their parameters respectively and calculate the intermediate results for the next-round iteration.
%This process repeats until the optimization converges.
%As such, by encapsulating and distributing multiplication and non-linear operations to different layer of participants, we can remove the cryptographic implementations of these operations

\codename is designed to preserve privacy in a way that the \emph{honest-but-curious} participants, who have access to the sum of the intermediate results produced by local nodes and additional knowledge learned from the training iterations, are unlikely~(i.e., with a negligible probability) to reveal the raw data or the local model parameters of other participants.
As a side effect of removing the cryptographic implementations of multiplications, the adversary obtains the \emph{party knowledge} from training iteration~(detailed in Section~\ref{sec:party}). %of some unencrypted intermediate results.
We prove that with a sufficient rank of the training dataset ($\geq$ 32 that is common in real-world datasets), \codename achieves the desired privacy preservation.

Notably, \codename introduces none sacrifice to the accuracy of models and also supports a wide range of machine learning algorithms. Intuitively, our solution makes use of chain rules in calculus to decompose gradient descent optimization into computational primitives, and distributed them to the local node and aggregation node respectively. When they collaborate together, these primitives can be recombined to achieve the correctness of learning.
We prove such correctness guarantee of any algorithms that use gradient descent for optimization, including but not limited to linear regression, logistic regression, and a variety of neural networks.

\paragraph{Contributions}
 In general, our contributions can be summarized as follows.
\begin{itemize}
	\item \textbf{A Novel Privacy-preserving Collaborative Framework.}
	We propose a novel framework \codename for privacy preserving collaborative learning while enabling a wide range of machine learning algorithms and achieving high computation efficiency.
	In \codename, not only original data, but also trained parameters are kept locally to ensure both the data and the trained model be confidential.

	\item \textbf{Provable Privacy Preservation and Correctness Guarantee.}
	We prove the privacy preservation %\highlight{security} \baigd{Is this security or privacy}
	of \codename, demonstrating a negligible probability for corrupted parties of revealing either the original data or the trained parameters from other honest parties. %, conditioned on a sufficiently large rank of training dataset.
	We also ensure the learning results to be exactly same in \codename as it is in the traditional non-distributed framework to guarantee the correctness.

	\item \textbf{Experimental Evaluations.} We run experiments on real datasets showing the significant improvement of efficiency of \codename compared with the state-of-the-art MPC and HE algorithms.
	For example, \codename  achieves around $22.5$ minutes for a two-hidden-layer neural network to process all samples in the MNIST dataset~\cite{lecun-mnisthandwrittendigit-2010}, while it takes more than $81$ hours with a state-of-the-art MPC protocol SecureML~\cite{mohassel2017secureml}.
\end{itemize}

\paragraph{Organization}
The rest of the paper is organized as follows. We briefly introduce necessary backgrounds of gradient descent and additive secret sharing scheme in Section \ref{sec:background}, and we present our design of \codename in Section \ref{sec:design}. We then prove the privacy preservation of \codename in Section \ref{sec:security}, and demonstrate its correctness and provide a case study of recurrent neural network in Section \ref{sec:corr&case}.  The efficiency performance are illustrated in Section \ref{sec:performance}. Section \ref{sec:related} reviews related works, and some concluding remarks are given in Section \ref{sec:conclusion}.


==> chapters/intro3.tex <==
\section{Introduction}

The performance of machine learning largely relies on the availability of data.
To take advantage of massive data owned by multiple entities,
the collaborative machine learning has been proposed to enable two or more data owners to construct a joint model.
To address the privacy concerns arising from the collaboration,
many studies~\cite{chen2018privacy, wang2019scalable, gascon2017privacy, zhang2019pefl} have managed to provide \emph{data locality} by distributing learning algorithms onto data owners such that the data can be confined within their owners.
Despite this, their learning processes still entail sharing and synchronizing on the locally trained models
and intermediate outcomes that may imply privacy-sensitive information~\cite{melis2019exploiting}.
A model-inversion attack is able to restore training data merely from the trained models, as demonstrated by Fredrikson et al~\cite{fredrikson2015model}.
In addition, in the scenarios where the model itself represents intellectual property, e.g., in financial market systems, it is an essential requirement that the local models are kept confidential~\cite{papernot2016towards}.
 
To provide a supplementary, i.e., \emph{privacy-preserving synthesis \baigd{what is the correct term in machine learning?} \yanjun{I thought ``privacy-preserving synthesis" is appropriate in our context.} of the local models and intermediate outcomes}, differentially private mechanisms and cryptographic mechanisms can be employed.
The former~\cite{zheng2019bdpl, hagestedt2019mbeacon, abadi2016deep, song2013stochastic, shokri2015privacy , dwork2014algorithmic, hu2019fdml} usually entail adding noise on the model parameters %\replace{training data}{model parameters},\baigd{should be on the parameters?} 
causing loss in accuracy of the final models.
The cryptographic mechanisms such as Homomorphic encryption (HE)~\cite{chen2018privacy, marc2019privacy, sharma2019confidential} and secure multiparty computation (MPC)~\cite{ gascon2017privacy, gascon2016secure, liu2017oblivious, mohassel2017secureml, bonawitz2017practical}
are able to yield identical models as those trained on plaintext data, but is known to be limited by the significant computational or communicational overhead.

This work focuses on the practicability of the cryptographic solutions. 
We propose a lightweight framework named \codename for privacy-preserving collaborative learning.
Our main strategy is to dispense the homomorphic \emph{multiplication operations} and \emph{non-linear functions} on encrypted data, as they are far more costly in computation\remove{/communication}\baigd{I am not sure whether their communication cost is much higher. If I understand it correctly, communication cost is from multiple rounds of messages back and forth. This should be addressed by redesigning the way of distributing the learning algorithms.} \yanjun{Multiplication/non-linear functions in garbled circuits/GMW based MPC protocol is costly with respect to communication (not computation). And in HE, they are costly with respect to computation (not communication). Our work is exactly ``redesigning the way of distributing the learning algorithms'' to avoid such operation on encrypted data, as the agg only requires the sum of intermediate results produced by local nodes. In contrast, if sending the gradients p1, p2 or training data x1, x2 out to the agg like in MZ17 (IEEE s\&p 2017 paper), crypto multiplication and non-linear function is indispensable.} than the \emph{addition operations}~\cite{gentry2009fully,albrecht2018homomorphic,yao1986generate, goldreich2019play}.
To this end, we redesign the workflow of collaborative learning, which employs merely the homomorphic addition operations provided by \emph{additive secret sharing scheme}~\cite{bogdanov2008sharemind}, when synthesizing local models and intermediate outcomes. 
\codename adopts the two-layer architecture commonly used by previous work on privacy-preserving collaborative learning. 
This architecture includes a local node layer which comprises of participating data owners, and an aggregation server which can be untrustworthy.
Both of the raw data and local models are always kept within their owners, 
and the computation executed by the aggregation node \remove{is} only  \replace{associated} {relies on} \baigd{what does ``associate'' mean here} \yanjun{I revised it to ``relies on"} \remove{with} the \emph{sum} of the intermediate results generated by local nodes~(detailed in Section~\ref{sec:workflow}).
\highlight{As such, we achieve significant cost savings compared with state-of-art garbled circuits and GMW based MPC protocol.}\baigd{I don't feel this sentence is in a right place. The saving is on computation, communication, or both?}\yanjun{Compared to garbled circuits/GMW based MPC protocol, the saving is on communication.}

\codename is designed to preserve privacy in a way that the \emph{honest-but-curious} participants, who have access to the sum of the intermediate outcomes produced by the local nodes and additional knowledge learned from the training iterations, are unlikely~(i.e., with a negligible probability) to reveal the raw data or the \highlight{local model parameters of other participants}. \baigd{This is a bit confusing. Is the local model something that needs to be shared with other local nodes/aggregation server, or something that can be derived from the shared intermediate outcomes. In the former, it needs to be protected during the synthesis process; in the latter, it is not required during the synthesis, so remove it from previous paragrah, such as ``privacy-preserving synthesis of the local models and intermediate outcomes'' in paragraph 2.} \yanjun{I thought the sentence ``privacy-preserving synthesis of the local models'' is correct in our context. Though the parameter itself is always kept locally, the intermediate results which is computed from the local model, i.e., the  multiplication results on the parameter and the raw data, is actually required during the synthesis, and they need to be protected. What I meant to say here is, even with the sum of these intermediate results, the probability of deriving the original data or the local parameter is negligible. }
As a side effect of our redesigned workflow, the adversary obtains the \emph{party knowledge} from training iteration~(detailed in Section~\ref{sec:party}). %of some unencrypted intermediate results.
We prove that with a sufficient rank of the training dataset ($\geq$ 32 that is common in real-world datasets), \codename achieves the desired privacy preservation.

Notably, the new collaborative learning workflow in \codename introduces none sacrifice to the accuracy of models, and also supports a wide range of machine learning algorithms as previous work does~\cite{abadi2016deep, mohassel2017secureml, hu2019fdml}. Intuitively, our solution makes use of the chain rules in calculus to decompose gradient descent optimization into computational primitives, and to distribute them to the local nodes and the aggregation node respectively. 
When they collaborate together, these primitives can be recombined to achieve the correctness of learning.
We prove that such correctness is guaranteed for any algorithm that uses gradient descent for optimization, including but not limited to linear regression, logistic regression, and a variety of neural networks.

\paragraph{Contributions}
 In general, our contributions can be summarized as follows.
\begin{itemize}
	\item \textbf{A Novel Privacy-preserving Collaborative Framework.}
	We propose a novel framework \codename for collaborative learning. 
    It preserves privacy while enabling a wide range of machine learning algorithms and achieving high computation efficiency.
	\highlight{In \codename, not only original data, but also trained parameters are kept locally to ensure both the data and the trained model be confidential.}\add{Not only does \codename achieve the data locality as previous work does, but it also keeps the local models and intermediate outcomes confidential.} \baigd{please make it clear the things protected by \codename: local model? intermediate outcomes? final model?} \yanjun{Local model actually equals the final model when the training converges. Intermediate results produced by local nodes are kept confidential by the additive secret sharing scheme, but the sum of them will be sent to the agg, I just wonder if ``the sum of them" would be regarded as another ``intermediate results"? So would it be appropriate to just say `` but it also keeps the local models confidential". Also, if we just say ``local models" here, we might also only mention the ``local models" (instead of ``local models and intermediate outcomes") in the paragraph 2? How would you think?}

	\item \textbf{Provable Privacy Preservation and Correctness Guarantee.}
	We prove the privacy preservation %\highlight{security} \baigd{Is this security or privacy}
	of \codename, demonstrating a negligible probability that corrupted parties are able to reveal either the original data or the trained parameters from other honest parties. %, conditioned on a sufficiently large rank of training dataset.
	We also prove that \codename ensures the learned model is identical as that in the traditional non-distributed framework.

	\item \textbf{Experimental Evaluations.} We run experiments on real datasets, showing that \codename achieves a significant improvement of efficiency over the state-of-the-art cryptographic solutions based on MPC and HE.
For example, \codename  achieves around $22.5$ minutes for a two-hidden-layer neural network to process all samples in the MNIST dataset~\cite{lecun-mnisthandwrittendigit-2010}, while it takes more than $81$ hours with a state-of-the-art MPC protocol SecureML~\cite{mohassel2017secureml}.
\end{itemize}

\paragraph{Organization}
The rest of the paper is organized as follows. We briefly introduce necessary backgrounds of gradient descent and additive secret sharing scheme in Section \ref{sec:background}, and we present our design of \codename in Section \ref{sec:design}. We then prove the privacy preservation of \codename in Section \ref{sec:security}, and demonstrate its correctness and provide a case study of recurrent neural network in Section \ref{sec:corr&case}.  The efficiency performance are illustrated in Section \ref{sec:performance}. Section \ref{sec:related} reviews related works, and some concluding remarks are given in Section \ref{sec:conclusion}.


==> chapters/related.tex <==
 \section{Related Work}
\label{sec:related}
%In this section, we review the existing privacy-preserving techniques which are divided into the following categories:
%Here, we review the most relevant techniques which are divided into the following categories:

Several works have been proposed for multiple entities to train machine learning models on their joint data without revealing any information beyond the outcome via HE or MPC solutions \cite{kwabena2019mscryptonet, zhang2017private, esposito2018securing, yuan2014privacy, hardy2017private, sadat2017safety, gilad2016cryptonets}. Recent studies \cite{gascon2017privacy, gascon2016secure}  propose a hybrid multi-party computation protocol for securely computing a linear regression model. %In \cite{yuan2014privacy}, a secure protocol is presented to calculate the delta function in the back-propagation training.
In \cite{liu2017oblivious}, an approach is proposed for transforming an existing neural network to an oblivious neural network supporting privacy-preserving predictions. However, cryptographic protocols may be not applicable to complex computation. For example, a MPC-friendly alternative function is specifically designed to replace non-linear sigmoid and softmax as the division and the exponentiation in these function are expensive to compute on shared values \cite{mohassel2017secureml}. Another well-known issue of traditional cryptographic protocols, as aforementioned, is the significant computational or communicational overhead.

In \codename, we do not require extra computational costs for computing the non-linear functions, so that functions like sigmoid and softmax can be used in training models as usual. In addition, the communication complexity is linear in the number of local nodes which is far more efficient than the traditional cryptographic solutions.
%Note that \codename is different from the distributed deep learning framework \cite{wang2019scalable,ghadimi2014optimal} in which the parameter server (PS) architecture %that synchronizes parameter updates (i.e., gradients) among multiple nodes
% is used, and the whole gradients are shared among the nodes. As a result, an attacker is able to infer the whole training data by compromising any parameter server in the system. In contrast, in our proposed framework, the corresponding gradients with respect to each data fragment are maintained in the local nodes separately for the purpose of privacy preservation.

Other than \cite{mcmahan2016communication} which focus only on preserving the privacy of training data, but the trained models are published to everyone, several recent works also pay attention to the privacy issues of the trained model. For example, \cite{papernot2018scalable} makes use of transfer learning in combination with differential privacy to learn an ensemble of ``teacher" models on data partitions, and then use these models to train a private ``student" model. However, these are centralized differential privacy mechanisms with a trusted aggregator. In contrast, in our framework, the aggregation server is not necessarily to be trustworthy.

The most related works to us are \cite{jia2016privacy,zhang2019enabling, zheng2019towards}, which have explored collaborative learning without exposing their trained models. Among these works, \cite{zheng2019towards} also exploits the lightweight additive secret sharing scheme for secure outsourcing of machine learning classification. However, their schemes only support specific algorithms, like support vector machine (SVM) in \cite{jia2016privacy}, summary statistics in \cite{zhang2019enabling} and decision tree in \cite{zheng2019towards}. %Therefore, new approaches need to be developed to support a wider range of functionalities.

